DALock: Distribution Aware Password Throttling

Large-scale online password guessing attacks are wide-spread and continuously qualified as one of the top cyber-security risks. The common method for mitigating the risk of online cracking is to lock out the user after a fixed number ($K$) of consecutive incorrect login attempts. Selecting the value of $K$ induces a classic security-usability trade-off. When $K$ is too large a hacker can (quickly) break into a significant fraction of user accounts, but when $K$ is too low we will start to annoy honest users by locking them out after a few mistakes. Motivated by the observation that honest user mistakes typically look quite different than the password guesses of an online attacker, we introduce DALock a {\em distribution aware} password lockout mechanism to reduce user annoyance while minimizing user risk. As the name suggests, DALock is designed to be aware of the frequency and popularity of the password used for login attacks while standard throttling mechanisms (e.g., $K$-strikes) are oblivious to the password distribution. In particular, DALock maintains an extra "hit count" in addition to "strike count" for each user which is based on (estimates of) the cumulative probability of {\em all} login attempts for that particular account. We empirically evaluate DALock with an extensive battery of simulations using real world password datasets. In comparison with the traditional $K$-strikes mechanism we find that DALock offers a superior security/usability trade-off. For example, in one of our simulations we are able to reduce the success rate of an attacker to $0.05\%$ (compared to $1\%$ for the $10$-strikes mechanism) whilst simultaneously reducing the unwanted lockout rate for accounts that are not under attack to just $0.08\%$ (compared to $4\%$ for the $3$-strikes mechanism).

==> MainAlgorithm.tex <==
\section{The DALock Mechanism}
In this section, we present the DALock mechanism, discuss how DALock might be implemented and the strategies that an attacker might use when DALock is deployed.

\subsection{DALock}
We formally introduce our main algorithm, DALock, in this section. We start by defining and describing the general framework of DALock. Following by proving why it is secure and user-friendly.

We first formally define classic throttling mechanism. Traditional Throttling mechanism maintains a counter k for each user u. Counter k stores consecutive incorrect login attempts in history. Typically, k is reset to 0 whenever u logins successfully. Some systems also reset k to 0 after a certain amount of time or maintain separate counters for different IP addresses. Mathematically speaking, one can define classic throttling mechanism as follows

\begin{definition}[($K$-Secure Throttling Mechanism]
Given integer K $\ge $ 1, $K$-Secure Throttling Mechanism $\mathcal{M}$ prevents login if $k \ge K$.
\end{definition}

DALock\ maintains extra ``hit count" $\psi$ corresponding to the total population density of attempted passwords. For example, if three incorrect passwords ``aaa"(3\%), ``bbb"(1.7\%), and ``lccc"(0.8\%) are attempted, then $\psi$ is set to 0.055.

\begin{definition}[($(\Psi, K)$-Secure Throttling Mechanism]
Given $\Psi > 0$ and  integer $k$ $\ge $ 1, $(\Psi, K)$-secure throttling mechanism $\mathcal{M}$ prevents login if
\begin{center}$k \ge K$ or $\psi \ge \Psi$\end{center} 
\end{definition}

We demonstrate the login flow in \textbf{Algorithm}~\ref{algo: login}. The pseudo code is self-explanatory, therefore we omit the detail description of it.

\begin{algorithm}[!htb]
	\caption{\textbf{DALock}: Novel Password Distribution Aware Throttling Mechanism }\label{algo: login}
	\textbf{Input: } Username $u$ and password $p$
	\begin{algorithmic}[1]
		\Function{login}{$u, p$} 
		\If {$\psi \ge \Psi$ or k $\ge$ K }
			\State Reject Login
		\EndIf
		\If{$p == u_p$}
			\State Reset k and $\psi$
			\State Grant Access
		\Else
			\State $\psi \leftarrow \psi + popularity(p)$
			\State $k \leftarrow k + 1$
			\State Deny Access
		\EndIf
		
	    \EndFunction
	\end{algorithmic}
\end{algorithm} 

\subsection{Implementing DALock}

To efficiently run DALock, one needs an efficient data structure to accurately, privately, and securely estimate the population density of passwords. We adopt Differential Private Count-Median-Sketch to store password distribution as it meets all the expectations. Due to space limitation, we omit the description of applying differential privacy to focus on discussion Count Sketch.

\begin{definition}[Count Sketch\cite{cormode2005improved}~\cite{charikar2002finding}]A Count sketch with volume V = w$\cdot d$ is represented by a two-dimensional array with width w and depth d. Additionally, it contains d + 1 hash functions
\begin{center}
$h_1 \cdots h_d$ : $\{\sigma^*\} \rightarrow \{1\cdots w\}$\\
$h_{\pm} : \{\sigma^*\} \rightarrow \{1, -1\}$\\
\end{center}
are chosen uniformly at random from a pairwise-independent family. Finally an integer T is maintained to record the total frequency.
\end{definition}
A typical Count Sketch involves the following operations:
\mypara{Add($p$):} Given input password word $p$ = $\sigma^*$, CS updates the table as follows: 
\begin{center}$\forall i \in d$, $CS[i,h_i(p)] \leftarrow CS[i,h_i(p)] + h_{\pm}(p)  $ \\ $T \leftarrow T + 1$  
\end{center}
\mypara{Estimate($p$):} Given input password word $p$ = $\sigma^*$, CS estimates its popularity based on predefined mechanism. 

In this work, we consider three popular estimation functions: Median, Mean, and Min. Median approach estimate the frequency of $p$ by $Median_{\forall i \in d}$( $CS[i,h_i(p)]\cdot h_{\pm}(p))$. Similarly, the other two approach use the mean and min of d values as estimation. 

 We discovered that Count-Median-Sketch outperforms Count-Mean-Sketch and Count-Min-Sketch for storing password distribution. In addition, we discovered that setting $d$ to 1 yields the lowest $l_1$ error for all CS. Subject to the space limitation, we only present the high level proof for Count-Median Sketch. 

\begin{theorem}[Optimal Parameter Choice of Count Sketch]
Given volume size V =  $d \cdot w$, the optimal choice of Count Sketch, Count Mean Sketch, and Count Min Sketch is to set $d$ = 1 when passwords follow Zipf's Distribution.
\end{theorem}
\mypara{Intuitive Proof:} 
Due to the nature of Zipf's distribution, the frequency count of any index CS[i,j] of a count median sketch is dominated by the most popular password hashed into that index. With larger d, an infrequent password p is more likely to collide with significantly more popular passwords on every row. Taking the median of d rows is essentially taking the median of d different popular passwords. Therefore, infrequent passwords are overwhelmingly overestimated with large d. 

\subsection{Attacker's Strategies}
In order to launch optimal dictionary attacks, $\mathcal{A}$ needs to find a subset of passwords that maximize its chance of success \textbf{without} triggering DALock. We proved this is computational challenging. In fact, it is $\NP$ hard to find the optimal guessing arrangement.

\mypara{Hardness of Password Cracking}
Perform optimal dictionary attacks on$(\Psi, K)$-Secure throttling mechanism is $\NP$ hard.

To maximized its chance of success, $\mathcal{A}$ has to select at most $K-1$ passwords from the dictionary s.t. the sum of popularity is maximized \textbf{and} not exceeding $\Psi$. This can be reduced to solving a well-known $\NP$ hard problem: Knapsacks. 

Admittedly, $\mathcal{A}$ can solve Knapsacks efficiently with close approximation because Knapsacks $\in \FPTAS$. Fortunately, users' unpredictable mistakes make the attack harder. $\mathcal{A}$ is forced to make a decision about how much  ``mistake budget"$\psi'$ to be reserved for users' potential mistakes.

Creating false popular passwords is another way to exploit DALock. In this circumstance, $\mathcal{A}$ needs to sign up sufficiently many accounts with infrequent passwords to decrease the popularity of true ones. Despite the fact that it can circumvent the restriction imposed by $\Psi$, $\mathcal{A}$ is still subject to counter $K$. Therefore $\mathcal{A}$ does not gain any advantage by disturbing distribution. 

%-----------BELOW NOT IN WAY--------------%
\begin{comment}
{\color{red} once again the statement is too informal to be place in a "lemma" environment. I would simply have informal discussion here.}
\begin{lemma}[Lower Economic Value of Password Cracking ]
Password Cracking under $(\Psi, K)$-Secure throttling mechanism yields lower economic value compare to $K$-Secure throttling mechanism.
\end{lemma}


\mypara{Intuitive Proof:} We prove that in both long term and short term attacks, $(\Psi, K$-Throttling mechanism decrease the profit of $\mathcal{A}$ by significantly delaying the guessing progress. 

We define one ``round" of attack as password guessing between a user's two successful login. Since successful logins reset cumulative thresholds $\psi$ and $k$, and users are likely to login regularly for online services. $\mathcal{A}$ can launch long-term online attacks to achieve higher economic gains. $\Psi$ naturally serves as an (overestimated) upper-bound on the potential economic gain for each round. We argue that there are two factors make the guessing a lot harder than $K$-Secure throttling mechanism.
\end{comment}
 

\begin{comment}
\mypara{Deferred High Quality Guess.} Let $\mathcal{A}$ be powerful that $\mathcal{A}$ can not only solve the t-round knapsack problem efficiently. In addition, assume $\mathcal{A}$ magically foresees future ``login patterns" of all users. $\mathcal{A}$'s maximum economic gain is still capped at $\Psi$. If most worth-to-try passwords have higher popularity density than $\frac{\Psi}{K}$, then $\mathcal{A}$ is significantly slowed down as $\mathcal{A}$ can't make k guess each round compare to $K$-Secure throttling mechanism. 
 \qed

\mypara{Users' Utility} Based on our empirical measurements, we discovered that $(K, \Psi)$-Secure throttling mechanism grants higher utility for users. Typos are generally very rare passwords. As a result, users can fully utilize $K$ attempts. We empirically demonstrates the result in \textbf{Section}~\ref{sec:oneroundexp}.
\end{comment}
%-----------ABOVE NOT IN WAY--------------%





\begin{comment}
\section{Results}\label{sec:main}
In this section, we present DALock mechanism and other results. Due to the space limitation, we present ``intuitive proof" of theorems instead of complete proof. In addition, we omit the discussion of how to compute and store frequencies of passwords privately. But keep in mind differential privacy\cite{dwork2011differential}, a mathematical rigorous and industry golden standard tool, has been used in our work.
\subsection{Optimal Size Choice of Count Sketch under Zipf's Distribution}
A Count sketch\cite{cormode2005improved}~\cite{charikar2002finding} with volume V = w$\cdot d$ is represented by a two-dimensional array with width w and depth d. Additionally, it contains d + 1 hash functions
\begin{center}
$h_1 \cdots h_d$ : $\{\sigma^*\} \rightarrow \{1\cdots w\}$\\
$h_{\pm} : \{\sigma^*\} \rightarrow \{1, -1\}$\\
\end{center}
are chosen uniformly at random from a pairwise-independent family. Finally an integer T is maintained to record the total frequency.



We omit the discussion of Count-Mean-Sketch and Count-Min-Sketch due to space limitation and similarity to Count-Median-Sketch.

\begin{theorem}[Optimal Size Choice of Count Sketch]
Given volume size V =  $d \cdot w$, the optimal choice of Count Sketch, Count Mean Sketch, and Count Min Sketch is to set $d$ = 1 when the dataset follows Zipf's Distribution.
\end{theorem}

\mypara{Intuitive Proof:} We present the high level idea of the proof for Count-Median Sketch only due to space limitation and similarity in proof for the rest two data structures.
\begin{comment}
Given total volume size V and a dataset $\mathcal{P}$ that follows Zipf's distribution. What's the optimal setting of $d$ and $w$ for CS i.e. one needs to solve the following integer programming problem
\begin{center}
	minimize $\displaystyle{\sum_{\forall p \in \mathcal{P}} |CS^{d,w}.Estimate(p) - F(p)|}$ \\
	subject to $d\cdot w$ = V\\
\end{center}
Where $SC^{d,w}$ is a SC with d rows and w columns, F(p) is the ground truth frequency of password p.
\end{comment}


\begin{comment}
\mypara{Proof:}
We start the proof by first formally formulating the question; Given total volume size V and a dataset $\mathcal{P}$ that follows Zipf's distribution. What's the optimal setting of $d$ and $w$ for CS i.e. one needs to solve the following integer programming problem
\begin{center}
	minimize $\displaystyle{\sum_{\forall p \in \mathcal{P}} |CS^{d,w}.Estimate(p) - F(p)|}$ \\
	subject to $d\cdot w$ = V\\
\end{center}
Where $SC^{d,w}$ is a SC with d rows and w columns, F(p) is the ground truth frequency of password p.

Given any password p, the estimation of its frequency from $CS^{d,w}$ is
\begin{align*}
CS^{d,w}.Estimate(p) &= median_{\forall i \in d}\{ CS[i,h_i(p)]\cdot h_{\pm}(p) \}
\end{align*}
Let $p_i$ be the set of passwords s.t. $\forall p' \in p_i$, $h_i(p') = h_i(p)$. i.e. $p_i$ is the set of passwords that has collision on $i^{th}$ row with p. Then the above formula can be rewritten as 
\begin{align*}
CS^{d,w}.Estimate(p) &= median_{\forall i \in d}\{ \displaystyle{\sum_{\forall{p' \in p_i}}F(p')\cdot h_{\pm}(p') }\}\\
\end{align*}

Let m the be index of row s.t. $CS[m, h_m(p)]$ is the median value across all rows. Then the estimation of p is 
\begin{align*}
CS^{d,w}.Estimate(p) & = CS[w, h_w(p)] \\
&= \displaystyle{\sum_{\forall p' \in p_m}F(p')\cdot h_{\pm}(p')}\\
&= \displaystyle{\sum_{\forall p' \in p_m}\frac{N}{2^{rank(p')}}\cdot h_{\pm}(p')}\\
\end{align*}
let $p^*$ be the one with highest frequency in  $CS[w, h_w(p)]$, let $F^*$ be the frequency of $p^*$
\begin{align*}
= \displaystyle{\sum_{\forall p' \in p_m}\frac{F^*}{2^{rank(p^*) - rank(p')}}\cdot h_{\pm}(p')}\\
= \displaystyle{F^*\sum_{\forall p' \in p_m}\frac{1}{2^{rank(p^*) - rank(p')}}\cdot h_{\pm}(p')} \\
\end{align*}
When $h_{\pm}(p^*) = 1$, 
\begin{align}
\displaystyle{E(\lim_{|p_m|\rightarrow \infty} CS^{d,w}.Estimate(p) )} \label{equation: rv} &= F^*\cdot(1 + 0)
\end{align}
Similarly, When $h_{\pm}(p^*) = -1$,  the expected value of the above sum is -1$\cdot F^*$. Notice that when the sign of $p^*$ is fixed, we can treat the rest $h_{\pm}(p')$ as Bernoulli random variables. For each random variable, it's expected value is 0 therefore the expected value of sum is the sum of expected values, which is 0. In fact, one can treat \textbf{Equation} ~\ref{equation: rv} as a uniform random variable ranges from [$0, 2\cdot F^*$] when , we plot the distribution in \textbf{Figure} ~\ref{fig: rv_plus.png}.
\end{comment}



\begin{comment}

\begin{figure}[htb]
\begin{center}
\includegraphics[height=2in,width=\linewidth]{figures/mainAlgo/DWTradeOff/plus.png}
\caption{PDF of equation ~\ref{equation: rv}  }\label{fig: rv_plus.png}
\end{center}
\end{figure}

\begin{figure}[htb]
\begin{center}
\includegraphics[height=2in,width=\linewidth]{figures/mainAlgo/DWTradeOff/minus.png}
\caption{PDF of equation ~\ref{equation: rv} (negative version)  }\label{fig: rv_minus.png}
\end{center}
\end{figure}

Notice that the above is the expected value of $CS[w, h_w(p)] $, or the estimated frequency of p. Let the rank of p be r, then probability of a password p becomes $p^*$ can be calculated as follows
\begin{align}
	\Pr{p* = p} &= \frac{\binom{|\mathcal{U}| - r}{\frac{|\mathcal{U}|}{w} - 1 }}{\binom{|\mathcal{U}| - 1 }{\frac{|\mathcal{U}|}{w} - 1 }}  \label{equation: wr_relation}
\end{align}
\textbf{Equation} ~\ref{equation:wr_relation} gives us the probability of p ``dominates" row i. If we want p to be comes median of d rows, the probability becomes $\frac{1}{d}$, therefore, getting correct estimation of p is 
\begin{align}
	\Pr{median = p} \frac{\binom{|\mathcal{U}| - r}{\frac{|\mathcal{U}|}{w} - 1 }}{\binom{|\mathcal{U}| }{\frac{|\mathcal{U}|}{w} - 1 }} \frac{1}{d} \label{equation: wdr_relation}
\end{align}
\textbf{Equation}~\ref{equation: wdr_relation} gives us the probability of a password p got correct estimation as a formula of w, d, and r. Thus, to increase the probability, one shall decrease d strictly.  
\end{comment}
\begin{comment}


Due to the space limitation, we omit the detail proof for Count Mean Sketch and Count Min Sketch. Instead, we demonstrate empirical results in \textbf{Section}~\ref{sec:dwtradeoff} . For curious readers, one can follow the above proof by making necessary changes to the above proof flow. Intuitively, when one sum d different $p^*$ values, $p^{**}$, the largest value among them, dominate the sum and therefore dominate the averages. 
\end{comment}


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> NewExperiment.tex <==

\subsection{Results on Subsampling}
We found that it is possible to deploy $\DALock$ without full dataset set based on our subsampling experiments. We remind readers that in such experiment, we implement $\DALock$ with Count Sketch $\sigma_{r\%}$ which is constructed based on sampling r\% of the users from true distriubiton. The results suggest that $\sigma_{r\%}$ can be as effective as $\sigma$ which indicates service providers do not need to collect an enourmous amount of data to implement $\DALock$.

One can observe such effects by comparing curves $\sigma_{1\% dp}$: CS-1\%(k:10,$\Psi:2^{-9.375},\epsilon$:0.1), $\sigma_{5\%}$: CS-5\%(k:10,$\Psi:2^{-9.375},\epsilon$:$\infty$) and $\sigma_{10\%}$: CS-10\%(k:10,$\Psi:2^{-9.375},\epsilon$:$\infty$) with $\sigma$: CS-all(k:10,$\Psi:2^{-9.375}$,$\epsilon:\infty$) from \textbf{Figure}~\ref{figure:dictionaryAttack9.375} and \ref{figure:usability9.375}. (Similarly for $\Psi = 2^{-7.0}$ from \textbf{Figure}~\ref{figure:dictionaryAttack7.0} and ~\ref{figure:usability7.0}.). Our results clearly demonstrates that of $\sigma_{1\%}$, $\sigma_{5\%}$, and $\sigma_{10\%}$ all have comparable performance with respect to $\sigma$ in both security and usability. 

\subsection{Results on Differentially Private Count Sketch}
Consider $\sigma_{1\%dp}$ mentioned in the previous section is a differentially private Count Sketch as well. Notice that for popular password pw, $\TrueFInD{pw}{\SampledData{\AllUser_{1\%}}}$ are roughly 100 times smaller compare to $\TrueFInD{pw}{\SampledData{U}}$ because of subsampling. Similarly, $\TotalFreq{\SampledData{U}} \approx 100\times \TotalFreq{\SampledData{\AllUser_{1\%}}}$. As a result, applying differential privacy to $\sigma_{1\%}$ produce more noisy results. Our experimental results on $\sigma_{1\%dp}$ show that it's performance is close to $\sigma$ in terms of both usability and security. This results suggest that with a reasonably large dataset, it's possible to deploy differentially private $\DALock$ with low privacy budget.

\subsection{Results on Other Estimators}
In this section we demonstrate our findings on implementing $\DALock$ with other estimators. We considered the following password strength meters: $\ZXCVBN$\cite{USENIX:Wheeler16}, Probablistic Context Free Grammar(PCFG), Neural Network, and Hashcat. The later four estimators are provided by Password Guessing Service\cite{USENIX:USBCCKKMMS15}. Since PGS also highly recommends use a hybird approach which takes the min guessing number of the later four apporaches to estimate the strength of passwords, we also include such methodology in our experiments. 

\noindent\textbf{Remark}: We omit the experiment results on Yahoo! for this part as password strength meters estimate the strength of passwords based on their string content. 

We discovered that it is feasible to deploy $\DALock$ with the above estimators; however, deploying them with an inapporiate $\hitCountThreshold$ can yields less demanding results. The experiments results can be found in \textbf{Figure}~\ref{figure:dictionaryAttack9.375}, \ref{figure:usability9.375}, ~\ref{figure:dictionaryAttack7.0}, and ~\ref{figure:usability7.0}. Based on the plots, we found PCFG and $\ZXCVBN$ have satisfying performance by setting $\hitCountThreshold = 2^{-9.375}$. Similarly Min, Markov, and Hashcat outperform 3-strike mechanism on both security and usability when $\hitCountThreshold$ is set to $2^{-7}$. We also found it's not possible to implement the estimator with Neural Netowrk (provided by PGS) alone as it regards most passwords as infrequent ones. 

\subsection{Results on Banning Popular Passwords}
We elaborate our findings on implement $\DALock$ with $\sigma_{-10000}$. Recall that $\sigma_{-10000}$ is constructed from the original dataset by banning top 10,000 passwords. In this scenario, the true distribution is flatend because of banning thus small $\hitCountThreshold$ is required to perform throttling. Our experimental results on $\hitCountThreshold$ = $2^{-11}$ can be found in \textbf{Figure}~\ref{figure:dictionaryAttackPrune} and ~\ref{figure:usabilityPrune}. 

Firstly, we found that dictionary attackers are strongly discouraged simply because of the distribution. By comparing \textbf{Figure}~\ref{figure:dictionaryAttackPrune} and \textbf{Figure}~\ref{figure:dictionaryAttack7.0}, one can observe that the compromised rates are significantly reduced. For example, the attacker can only compromise 1\% of users accounts on $\text{LinkedIn}_{-10000}$ while they can acheive 12\% on the original dataset. 

Secondly, we discoverd that Count-Sketch based $\DALock$ can be deployed on a flat distribution. By comparing curves $CS-all(K:10,\Psi: 2^{-11.0}, \epsilon)$ and 3-strike from \textbf{Figure}~\ref{figure:dictionaryAttackPrune}  and ~\ref{figure:usabilityPrune}. Despite the advantage on security side is minor, Count Sketch based $\DALock$ results in lower unwanted locked out rate. 

Thirdly, we do acknowledge that it is a challenging task to implement estimator with password strength meter under a flat distribution. Based on results, it's impossible to find a $\hitCountThreshold$ value such that one can beats 3-strike for both security and usability. 






==> SimulateUser.tex <==
% Comment Unwanted text for later S&p Submission
% !TEX root = main.tex
\section{Simulating Users' Login Activities} \label{sec:simulateUsers}
To accurately assess the performance of $\DALock$, it' crucial to simulate user's behavoir reasonbly.  In this Section, we focus on discussing how to simulate users' login activities in our experiments. Generally speaking, there are three aspects one needs to consider:
\begin{itemize}
	\item User's password choice.
	\item User's login patterns/frequency.
	\item User's Honest mistake
\end{itemize}



\subsection{Simulating Users' Choice of Password}

This is a straight forward task for RockYou dataset. Ideally, one can create users and assign passwords based on the distribution of plaintext password strings. In our simulation, a users' chance of selecting a particular password is identical to it's popularity density in the dataset. For example, When simulating experiments based on RockYou dataset, each user has probability 0.89\% to choose ``123456" as their password. 

\mypara{Simulating Password Choices on LinkedIn and Yahoo} It's tricky to simulate users' choice of password strings based on dataset \textbf{LinkedIn} and \textbf{Yahoo}as we don't have the plaintext of passwords. To overcome this issue, we map passwords from \textbf{RockYou} to \textbf{LinkedIn} and \textbf{Yahoo} as follows:

\begin{itemize}
	\item Map top 20,000 passwords from RockYou to top 20,000 passwords of LinkedIn/Yahoo
	\item Map rest of the passwords uniformly according to ranks.
\end{itemize}

For example, the most popular password from LinkedIn is represented by ``123456", the most frequent password from RockYou. The second most popular password from LinkedIn is ``12345" after mapping. The first 20,000 password strings will be exactly the same as top 20,000 passwords in RockYou. For the rest of the passwords, we either uses a random password string or uses a password string from RockYou. Since  RockYou has 14,341,564 uniques passwords and LinkedIn has 60,065,486 unique passwords, we map password string to LinkedIn from RockYou roughly every 4 passwords/ranks. 

We argue the above simulation is reasonable and valid. For attacker, this hardly makes any difference as they cares significantly more on password popularities ithan the content of the strings. On the other hand, the choice of password string can have a significant impact on users. For instance, users who choose ``123456" as their password are more likely to get locked out if they enter ``12345", the second most popular password in the dataset. Therefore, to simulate a proper distribution, we map passwords as we mentioned above.



\subsection{Simulating user's login patterns}Following prior work we use a Poisson arrival process to model a user's login activities\cite{AC:BloBluDat13}\cite{CCS:KogManBon17} with arrival rate parameter $t_u$ for each user u. To verify the performance of $\DALock$ over a reasonablly long time span, we simulate the login activities over time span of 180 days, or 4320 hours. In our simulation, each user's login activities can be viewed as a sequence of increasing random variables $0 < T_1 < t_2 < \cdots <  4320 = 180*24$. Each random variable T, or login activity, is generated from range 0 to 4320 to represent u' login activities at time R over 180 days time span (rounded to hours). The smaller value of $t_u$, the more frequent u logins into her accounts. To have a realistic representation of login pattern, for each user u, $t_u$ is sampled uniformly random from \{ 12, 24, 24 * 3, 24 * 7, 24 * 14, 24 * 30\}.

Notice that for each login activity, more than one login attempts can generated because of users' mistakes. Naturally, we simulate each login activity by assuming that users will keep trying until they successfully login into their account, or get locked out unfortunately.



\subsection{Simulating user's mistakes} is the last challenging ingredient for simulating user's login activities. In order to reasonably simulate user's mistakes, two major type mistakes were took into considerations: entering a different password or making typos on the original passwords. We followed a recently published statics on users's mistakes\cite{CCS:CWPCR17} to setup the probability of users' (varies type of) mistakes. Based on the results of the literatures, users have roughly 7.5\% chance of making a mistake (Pr(Mistake) = 0.075). Among those mistakes 68\% of those incorrect attempts are within editing distance 2. To simplify the model and analysis, we consider that as the probability as making typos. i.e. given a password p, user has probability $0.075\cdot 0.68$ of typing it wrong. We summarized the distribution of various types of typos in Table~\ref{Table:TypoTypes} for reader's convenience.  Further more, we consider the rest 32\% errors come from entering wrong passwords(editing distance greater than 2), in another word, entering different passwords. Therefore, each user has probability $0.075\cdot 0.32$ to select a wrong password to attempt (of course, the user can make typos on top of that!). We setup such secondary passwords (in users' mind) when users are created by randomly sampling a different password for each user based on the distribution of passwords. To help readers capture the essence of user's honest mistakes are simulated in our experiment, we present the flow chart in Figure ~\ref{fig:flowChartTypo}, \textbf{Appendix}.



==> cfp.tex <==
\section{Call for Papers}

The conference seeks submissions presenting novel research results in
all aspects of computer and communications security and privacy,
including both practical and theoretical contributions.

\subsection{Paper Submission Information}

Submissions must be received at \url{https://ccs17.hotcrp.com/} by the
strict deadline of {\bf 19 May 2017 at 8:59 PM PDT (UTC-7)}.
Submitted papers must not substantially overlap with papers that have
been published or that are simultaneously submitted to a journal,
conference, or workshop. Submissions must be anonymized and avoid
obvious self-references.

CCS has traditionally required that authors submitting papers
guarantee that an author will be able to present their paper at the
conference. We recognize, however, that the current travel
restrictions and screening processes may make it impossible or
uncomfortable for some authors to travel to the conference. The venue
for CCS 2017 was selected several years ago, and we do not wish to
exclude any potential authors who may have difficulty traveling due to
recent changes in US immigration practices.  CCS welcomes submissions
by authors of all nationalities, and will make allowances for
presenting papers electronically or with non-author presenters in
cases where paper authors are unable to travel to the United States.

Submissions will be evaluated based on their scientific merit,
novelty, importance, presentation quality, and relevance to computer
and communications security and privacy.  If a paper includes work
that raises ethical concerns it is up to the authors to convince the
reviewers that appropriate practices were followed to minimize
possible harm and that any harm caused by the work is greatly
outweighed by its benefits. The review process will be carried out in
two phases and authors will have an opportunity to provide a
length-limited response to the first-phase reviews.

\subsection{Paper Format}

Submissions must be single PDF files containing at most 12 pages in
the required new ACM format (see
\url{https://www.sigsac.org/ccs2017/format} for details and templates,
which you have presumably found if you are reading this!) of body
content, with any number of additional pages for the bibliography,
well-marked appendices, and any desired supplementary material.  When
relevant, submitters may include reviews from past submissions and
responses to them in the supplementary material.

Reviewers are not required to consider the appendices or supplementary
material, however, so submissions need to be intelligible and
convincing without them.  Submissions not meeting these guidelines, or
playing games to work around page limits, will be rejected by the PC
chairs without review.  In particular, papers should not use squeezing
tricks to adjust the (already very dense) ACM paper format, and moving
discussion of key related work or important definitions to appendices
may be grounds for rejection.

\subsection{Practice Talks}

Following the lead of USENIX Enigma, we want to improve the quality of
the conference and provide a better experience for both presenters and
attendees by holding practice sessions before the conference (see
\url{https://www.sigsac.org/ccs2017/practicefaq}). Presenting authors
of accepted papers are expected to participate in an on-line practice
session approximately three weeks before the conference.

\subsection{Conflicts of Interest}

The conference requires cooperation from both authors and program
committee members to ensure a process that is both fair in practice
and perceived to be fair by everyone. When submitting a paper, authors
are required to identify members of the program committee who may not
be able to provide an unbiased review.  This includes people with
strong personal or professional relationships such as advisor/advisee,
members of the same organization, and close collaborators (for
example, recent or repeated co-authors). In general, this means anyone
who a reasonable person with all the relevant information would
question as an impartial reviewer. The program co-chairs reserve the
right to request a more specific description of a conflict-of-interest
declaration from authors.

Program committee members who have a conflict of interest with a
paper, including program co-chairs, will be excluded from evaluation
and discussion of the paper, but because submissions are anonymous to
reviewers it is important for submitting authors to identify these
conflicts. In the case of a program co-chair, the other co-chairs who
do not have conflicts will be responsible for managing that paper.
Program co-chairs are not permitted to be involved as co-authors in
any submissions.



